Scalable Relational Query Processing on Big Matrix Data

The use of large-scale machine learning methods is becoming ubiquitous in many applications ranging from business intelligence to self-driving cars. These methods require a complex computation pipeline consisting of various types of operations, e.g., relational operations for pre-processing or post-processing the dataset, and matrix operations for core model computations. Many existing systems focus on efficiently processing matrix-only operations, and assume that the inputs to the relational operators are already pre-computed and are materialized as intermediate matrices. However, the input to a relational operator may be complex in machine learning pipelines, and may involve various combinations of matrix operators. Hence, it is critical to realize scalable and efficient relational query processors that directly operate on big matrix data. This paper presents new efficient and scalable relational query processing techniques on big matrix data for in-memory distributed clusters. The proposed techniques leverage algebraic transformation rules to rewrite query execution plans into ones with lower computation costs. A distributed query plan optimizer exploits the sparsity-inducing property of merge functions as well as Bloom join strategies for efficiently evaluating various flavors of the join operation. Furthermore, optimized partitioning schemes for the input matrices are developed to facilitate the performance of join operations based on a cost model that minimizes the communication overhead.The proposed relational query processing techniques are prototyped in Apache Spark. Experiments on both real and synthetic data demonstrate that the proposed techniques achieve up to two orders of magnitude performance improvement over state-of-the-art systems on a wide range of applications.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
		Corrected the bug with acmPrice.
		Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
		The package now is compatible with polyglossia (Joachim Breitner).
		Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
		Deleted indent for subsubsection (suggested by Ross Moore)
		Suppressed some obscurious warning in BibTeX processing
		Suppressed hyperrerf warnings (Paolo G. Giarrusso)
		New code for sections to help with accessibility patches
		(Ross Moore)
		Submission id, if present, is printed in anon mode
		Bug fixes

Version 1.55    Bug fixes


==> figs/impl.tex <==
\section{System Implementation}
%Mingjie: update the title since this is same as MatFast
\label{sec:impl}
After query execution plan and matrix data partitioning schemes are generated, each worker conducts matrix and relational computations locally.
\system~leverages block matrices as a basic unit for storing and manipulating matrix data in the distributed memory. We discuss briefly the system implementation on top of Spark SQL.

\subsection{Physical Storage of a Local Matrix/Tensor}
\label{physical-storage-matrix}
We partition a matrix into smaller square blocks to store and manipulate matrix data in the distributed memory. The smaller blocks can better utilize spatial locality of nearby entries in a matrix. A matrix block is the basic unit for storage and computation. Figure~\ref{fig:block_matrix} illustrates that Matrix $\mA$ is partitioned into blocks of size $3 \times 3$, where each block is stored on a worker locally. 
For simplicity, we only consider square blocks. To fully exploit modern CPU cache size, \system~sets block size to be 1000.

Every matrix block consists of two parts: a block ID and matrix data. 
A block ID is an ordered pair, i.e., (row-block-ID, column-block-ID). The matrix data field is a quadruple, $\langle$matrix format, number of rows, number of columns, data storage$\rangle$.
A local matrix block supports both dense and sparse matrix storage formats.
For the sparse format, the nonzero entries are stored in Compressed Sparse Column~(CSC), and Compressed Sparse Row~(CSR) format.
More details of local matrices are discussed in~\cite{matfast}.

A join may produce a normal matrix or a higher-dimensional tensor, e.g., a 3rd-order tensor for joins on a single dimension. \system~utilizes block matrices to manipulate higher-dimensional tensors as well. 
Given a 3rd-order tensor, the schema of the tensor is represented as \texttt{(D1, D2, D3, val)}, where \texttt{D1}, \texttt{D2}, and \texttt{D3} denote the three dimensions. 
To leverage the block matrix storage, \system~extends the block ID component to higher dimensions, e.g., (D1, D2-block-ID, D3-block-ID), where D1 records the exact dimension value, and the remaining record the matrix block IDs for the other dimensions.
Figure~\ref{fig:block_tensor} illustrates the storage layout of a 3rd-order tensor in terms of matrix blocks.
There is freedom on choosing which dimension of the tensor to serve as D1, D2, or D3. 
Usually there exits an aggregation  on a certain dimension following the join. A heuristic is to choose a non-aggregated dimension as D1 in a physical block storage.
It is beneficial that each worker only needs to execute the aggregation locally without further communication.
Figure~\ref{fig:block_tensor} demonstrates 2 possible tensor layouts on dimension D1 and D3 respectively.
If a subsequent aggregation is performed on dimension D2 or D3, \system~stores the join result in block matrices with respect to dimension D1. %Any aggregation on D2 or D3 can be simply executed independently on each worker.
\begin{figure*}[!ht]
%\vspace{-0.5em}
\centering
\begin{subfigure}{\columnwidth}
\includegraphics[width=0.88\columnwidth]{./figs/matrix_storage_matrel}
\caption{Block matrix storage}
\label{fig:block_matrix}
\end{subfigure}\hfill
\begin{subfigure}{\columnwidth}
\includegraphics[width=0.88\columnwidth,height=4cm]{./figs/tensor_storage}
\caption{Block tensor storage}
\label{fig:block_tensor}
\end{subfigure}
\caption{Physical storage of block matrix and tensor.}
\vspace{-1em}
\label{fig:physical_storage}
\end{figure*}

% \subsection{Local index on the cell values of a matrix/tensor}
% Discuss about the proposed \textit{learned index} on the matrix data. The index is essentially a function that maps a cell value to a set of (rid, cid). We cannot learn a one-to-many mapping. Have to come up with an intelligent encoding to wrap the set into a single ``number''.

\subsection{System Design and Implementation}
\system~is implemented as a library in Apache Spark. It extends Spark SQL and its Catalyst optimizer to work seamlessly with matrix/tensor data. We provide Scala API for conducting relational query processing on distributed matrix data. It uses a DataFrame~\cite{sparksql} to represent distributed matrix blocks. Each row in a DataFrame has the schema \texttt{(RowBlkID, ColBlkID, Matrix)}, where both IDs takes a long integer type, and \texttt{Matrix} is a user-defined type that encodes the quadruple shown in Figure~\ref{fig:block_matrix}.
For logical optimization, we extend the Catalyst optimizer with all the transformation rules for optimizing the relational operations on matrix data.
Once an optimized logical plan is produced, \system~generates one or more physical plans. By leveraging the cost model for communication, the matrix data partitioner selects the partitioning schemes for input matrices, that incurs minimum communication overhead. Finally, the optimized physical plan is realized by RDD's transformation operations, e.g., \texttt{map}, \texttt{flatMap}, \texttt{zipPartitions}, and \texttt{reduceByKey}, etc. The RDD partitioner class is extended with three partitioning schemes for distributed matrices, i.e., Row, Column, and Broadcast. 
Spark's fault tolerance mechanism applies naturally to \system. In case of node failure, the lost node is evicted and a standby node is chosen to recover the lost one.
An open-source version of \system~is available on GitHub\footnote{\url{https://github.com/yuyongyang800/SparkDistributedMatrix/tree/spark-2.1-dev}}.

==> figs/join.tex <==
\section{Join on matrix data}
The relational join~($\Join$) is a useful operator for picking corresponding entries that satisfy the join predicates from two separate matrices. For example, raster data overlay analysis~\cite{hadoopviz} requires a join on two matrices with matching row/column index, where a raster map can be interpreted as a matrix. 
%M: what is the meaning of raster analysis ? we do not know how it works as well? 
%Yongyang: Raster data is essentially represented by matrix.  We introduce join operation given raster data analysis as a motivation.
Formally, a relational join is a binary operator,
\[
\mA \Join_{\gamma, f} \mB,
\]
where $\gamma$ is the join predicate, $f$ is the user-defined merge function that takes two matching entries and outputs a merging result, e.g., $z=f(x,y)$. We introduce various formats of $\gamma$ in different semantics in the subsequent sections. In general, the result of a relational join on two matrices is a \emph{tensor}, or a multi-dimensional array, whose dimensions are determined by the predicate $\gamma$.
We first discuss how to infer the schema of a join output based on the join predicates. Next, we introduce all the valid formats of $\gamma$. Finally, we investigate the optimization strategies for join executions.



\subsection{Schema of the join result}
%The output of a join operation is generally a tensor. 
Just like every matrix has a schema, 
%M: what is the schema of matrix? 
%Yongyang: The schema is discussed in Section 3.1.1.
\system~automatically produces a schema for a join result. The schema of a join result consists of two parts: the index and the value. In this work, we only consider equality predicates as the join condition. Given two input matrices $A(RID_A, CID_A, val_A)$ and $B(RID_B, CID_B, val_B)$, the cardinality of the dimension of $\mA \Join_{\gamma, f} \mB$ is 
\[
d = 4 - \delta_{dim},
\]
where $\delta_{dim}$ is the number of equality predicates on the join dimensions. For example, if the join predicates $\gamma=``RID_A=RID_B"$, the join output boasts the schema $(D_1, D_2, D_3,val)$,
where $D_1$ takes matching dimension from $RID_A$, $D_2$ takes relevant dimension from $CID_A$, $D_3$ takes relevant dimension from $CID_B$, and $val$ is the evaluation of the merge function on the matching entries from $\mA$ and $\mB$. The join output may degrade to a normal matrix when $\gamma$ contains two or more predicates on the join dimensions.
%Mingjie: why 4-xxx? number of equality predicates on the join dimensions? do not know
%Yongyang: A matrix has two dimensions, row and col. Two matrices have 4 dimension in total. If there are k matching dimensions, then (4-k) dimensions are left to index any entry in the join result.

%The result may be a normal matrix or a high-dimensional tensor\\

%different types of join on matrix data\\

%we may need to express the matrix data in a relation, then perform joins on the relation to explain the meaning of the schema\\

%exploring the sparsity-preserving udf

\subsection{Cross-product on two matrices}
The cross-product operator is a special join operator between two matrices, where the join predicate $\gamma$ is empty, i.e.,
$\mA \kron \mB = \mA \Join_f \mB$.
If both input matrices are viewed as relations, 
this operator is essentially the Cartesian product.
The cross-product is widely used in tensor decomposition and applications, e.g., Kronecker product~\cite{Kolda:tensor}.
\system's optimizer infers the output schema from the join predicate, which is empty for cross-product. Therefore, a cross-product produces a 4th-order tensor from two input matrices. 
For example, $C(D_1, D_2, D_3, D_4, val)$ is the schema of $\tensor C = \mA \kron \mB$.
The first two dimensions $(D_1, D_2)$ inherit from $\mA$, and the last two dimensions $(D_3, D_4)$ inherit from $\mB$.


The execution of a cross-product is conducted in a fully parallel manner. \system~stores a matrix in blocks of equal size, where the blocks are distributed among all the workers in a cluster. First, each block of the smaller matrix  is duplicated $p$ times, where $p$ is the number of partitions from the larger matrix. Next, each duplicated block is sent to a corresponding partition of the larger matrix. Finally, each worker performs join operation locally without further communication. The 4th-order tensor is stored as a series of block matrices in a distributed manner. The detailed physical storage is described in Section~\ref{physical-storage-matrix}.
%Mingjie: you mix the computation and logical plan together, maybe you just need to say what is the output of cross-product result. 
%Yongyang: The output of a cross-product is a 4th-order tensor. The above paragraph describes the physical plan of cross-product execution.

\subsection{Join on two dimensions}
%Mingjie: you mention the overlap two matrix together, why it is two dimensions? 
%Yongyang：To compute an overlap of two matrices, one has to align both row and column dimensions, or join on the two dimensions.
The dimension-based predicates for join on two dimensions can take two different formats:
\[
\mA \Join_{RID_A = RID_B \land CID_A = CID_B,f} \mB,
\]
or 
\[
\mA \Join_{RID_A = CID_B \land CID_A = RID_B,f} \mB.
\]
These two predicates are the only valid formats, as a propositional formula takes dimensions from both inputs.
The former predicate can be viewed as an overlay on the two input matrices directly~(\textit{direct overlay}), while the latter can be viewed as an overlay on Matrix $\mA$ and the transpose of Matrix $\mB$~(\textit{transpose overlay}). Figure~\ref{fig:direct_overlay} illustrates an example of direct overlay. Conceptually, two input matrices can be regarded as two relations with the schema introduced in Section~\ref{section:schema}. The output of a join on two dimensions is a normal matrix, since two common dimensions are shared with the inputs. 
% We do not consider other variants of join predicates on the same matrix in \system. For example, 
% \[
% \mA \Join_{RID_A = CID_A \land RID_B = CID_B, f} \mB,
% \]
% since this kind of join predicates only involve entries within a single input matrix, which violates the definition of the merge function.

%join condition can be (r1 = r2 and c1 = c2, direction overlay) or (r1=c2 and r2=c1, transpose overlay), otherwise not make sense
\begin{figure}
\centering
\includegraphics[width=0.85\columnwidth]{./figs/matrix_join}
\caption{Direct overlay of two sparse matrices.}
\vspace{-1em}
\label{fig:direct_overlay}
\end{figure}

To efficiently evaluate joins on two dimensions, \system~adopts the hash join strategy to partition the matrix blocks from the inputs. By hashing the matched matrix blocks to the same worker, a worker conducts local join execution without further communications. For direct overlay, \system's planner partitions the two input matrices using the same partitioner. For transpose overlay, the planner makes sure the partitioning scheme on one input matches the partitioning scheme on the transpose of the other.


\subsection{Join on a single dimension}
The dimension-to-dimension~(D2D) predicates can take four different formats:
\[
\mA \Join_{ID_A = ID_B, f} \mB,
\]
where $ID_{A/B} \in \{RID_{A/B}, CID_{A/B}\}$.
Therefore, the join output is a 3rd-order tensor, and takes the schema $(D_1, D_2, D_3, val)$.
Each entry from a matched row/column from $\mA$ is joined with the entries from the corresponding row/column from $\mB$.
%This join operation can be leveraged as a building block to answer zonal queries.

\system~leverages a hash-based data partitioner to map matched row or column matrix blocks to the same worker. Suppose both input matrices are partitioned into $\ell$-by-$\ell$ square blocks. Let us consider the D2D predicate to be $``RID_A=RID_B"$. Two matrix blocks $\mA_{mp}$ and $\mB_{mq}$ are mapped to the same worker. For the $t$-th row from $\mA_{mp}$, each entry is joined with the same row from $\mB_{mq}$. Thus, a $1$-by-$\ell$ vector is produced by joining a single entry in the $t$-th row 
from $\mA_{mp}$ and an entire row from $\mB_{mq}$. 
After the join operation, the $t$-th row from $\mA_{mp}$ leads to an $\ell$-by-$\ell$ matrix block. 
%with the block ID $(m\ell+t, p, q)$, where $m\ell+t$ is the absolute ID of the first dimension, $p$ and $q$ are the block IDs of the second and third dimensions. 
Potentially, there are totally $\ell$ such matrix blocks for the join result from two input matrix blocks.


\subsection{Join on the entries}
The entry-based~(value-to-value, or V2V) join operation takes the following format:
\[
\mA \Join_{val_A = val_B, f} \mB.
\]
The join output is a 4th-order tensor, where the first two dimensions come from the dimensions of $\mA$, and the other two from the dimensions of $\mB$.

The execution of a V2V join is conducted in a fully parallel manner, similar to the execution of cross-product.
\system~broadcasts each block of the smaller input to each partition of the larger one.
Each worker in the cluster adopts a nested-loop join strategy to compute the join locally by taking each pair of matrix blocks. The four dimensions are copies of the dimension values from matched entries.% from the input matrices.

\subsection{Join on a single dimension and an entry}
The join on a single dimension and an entry operation~(D2V, or V2D) takes the following format:
\[
\mA \Join_{ID_A = val_B, f} \mB \text{, or } \mA \Join_{val_A = ID_B, f} \mB
\]
where $ID_{A/B} \in \{RID_{A/B}, CID_{A/B}\}$.
%From the perspective of relational algebra, there is one more valid format of join operation, join on a dimension and an entry value. 
The output is a 4th-order tensor, where the 4 dimensions derive from the entry locations of the matched rows/columns, and the matched entries from the other input. To evaluate this type of join, the matrix blocks containing the matched entries are mapped to the other matrix, where the row/column dimension matches. Each worker conducts local join computation based on the matched dimensions and entries.
%As this type of join is not commonly used in real-world applications, we do not discuss it in more details.
% \subsubsection{Join on an index and a cell value(keep it or drop it?)}

% the operation is valid from a relational algebra perspective; no good insight into why this is good for real-world applications\\
%  Results in a 4d-tensor

\subsection{Join optimization}
Relational joins over matrix data are more complex than other relational operations. They potentially have higher computation and communication overhead. We have identified several heuristics to mitigate the heavy memory footprint and computation burden. We leverage the following features: (1) sparsity-preserving merge functions, and (2) Bloom-join for join on entries. Furthermore, we also develop a cost model to capture the communication overhead among different joins. By utilizing the heuristics and the cost model, \system~generates a computation- and communication-efficient execution plan for a join operation.

\textbf{Identifying Sparsity-preserving Merge Functions.} Given a general join operation, $\mA \Join_{\gamma, f} \mB$, there are two important parameters, $\gamma$ and $f$. The predicate $\gamma$ is utilized to locate the join entries, and $f$ is evaluated on the two entries for an output entry. In real-world applications, large matrices are usually sparse and structured\footnote{\url{http://www.cise.ufl.edu/research/sparse}}. For example, Figure~\ref{fig:direct_overlay} illustrates a direct overlay on two sparse matrices, where the merge function is $f(x,y) = x + y$.
We say $f(x, y)$ is a sparsity-preserving function if $f(0, \cdot) = 0$ or $f(\cdot, 0) = 0$. Thus, the summation merge function is \textit{not} sparsity-preserving since $C_{00} = A_{00} + B_{00} = 0+2=2$, which does not preserve sparsity from the left- or right-hand side. On the other hand, $f_1(x, y) = xy$, is sparsity-preserving on both sides.

The benefit of utilizing sparsity-preserving function is obvious, as it avoids evaluating the function completely if one of the inputs contains all zeros.
Traditionally, a straw man execution plan takes two input matrix blocks. It at first converts the sparse matrix formats to the dense counterpart by explicitly filling in 0's, then evaluates the merge function on the matched entries. Note that a sparse matrix format only records nonzeros and their locations. Compressed sparse representations reduce memory consumption and computation overhead for matrix manipulations. However, the memory consumption grows significantly when a sparse matrix is stored in the dense format.
%Mingjie: confused the example here:  change the matrix to dense counterpart, but you said that dense part is not good. thus, what you want to say is that human drawn plan is bad comparing with your approach? you need to explain "dense counterpart", "compressed sparse representations" more clearly here. 
%Yongyang: For a naive approach, the merge function requires two matching entry values to compute a corresponding output. If the inputs are sparse matrices, then the naive approach has to convert the sparse format to the dense format to obtain the entry values, since the 0's are not explicitly stored in sparse formats. I try to illustrate the importance of the sparsity-preserving property of merge functions.

Thus, it is critical to identify the sparsity-preserving merge functions, and avoid converting a sparse matrix format to dense  format whenever possible. We consider a special family of merge functions: linear function and their linear combinations, i.e., 
$f(x,y) = g(x)y + h(x)$, or $f(x,y) = g(y)x + h(y)$, where both $g(\cdot)$ and $h(\cdot)$ are linear functions.
For any merge function in this family,
\system~adopts a sampling approach to identify the sparsity-preserving property. Given a merge function $f(x, y)$, we compute $t_1 = f(0, s_1)$, and $t_2 = f(0, s_2)$, where $s_1$ and $s_2$ are random numbers. If both $t_1$ and $t_2$ are 0, $f(x,y)$ is sparsity-preserving because of the linearity of function components. A similar sparsity-preserving test could be conducted on the $y$ value.

Once a sparsity-preserving function is identified, \system's planner orchestrates the execution of join operations by leveraging the sparse matrix computations. For example, if the merge function $f(x,y)$ boasts the sparsity-preserving property on the $x$ component, \system~only retrieves the nonzero entries from the left-hand side, and joins with entries from the right-hand side. All the computations are conducted in the sparse matrix format without converting to dense matrix format.
%Mingjie: what is the mean of orchestrates? 
%Yongyang: It's another way of saying "arranges" or "plans".

\textbf{Bloom-join on Entries.}
For a join predicate that involves a dimension on the matrix, it is efficient for \system~to locate the corresponding row matrix blocks or column matrix blocks. The irrelevant matrix blocks are not accessed during evaluation. However, the join operation becomes expensive when the join predicate contains a comparison on the entries. A straw man plan compares each pair of entries exhaustively, where a lot of computation is wasted on the mismatched entries.
%Mingjie: confused here as well. the straightforward approach is not well explained. 
%Yongyang: The straight-forward approach just enumerates each pair of entries from both inputs to compute an entry in the output. This is very inefficient if the entry value does not exist at all in one of the input. That's why we introduce Bloom-join for this situation.

\system~adopts a Bloom-join strategy when a join predicate contains matrix entries. Each worker computes a Bloom filter on the entries. Due to the existence of sparse matrices, a worker needs to determine whether to store 0's in the Bloom filter. Thanks to the heuristic of identifying zero-preserving merge functions, 0 values are not inserted into the Bloom filter if $f(x, y)$ is sparsity-preserving. After each matrix block creates its own Bloom filter, a worker picks an entry from one of the input matrix and consults the Bloom filter on the other input. If no match is detected from the Bloom filter, the join execution continues to the next entry; otherwise, a nested-loop join is conducted on the input matrices to generate the join output.
%Mingjie: maybe an example to help understand 


% heuristics:\\
% A straw man approach will convert both input blocks to dense matrices, and examine each pair of entries for testing the join predicates.\\

% bloom join on the values, to skip irrelevant matrix blocks; do we store 0's in the bloomfilter?\\

%build a ML model to compute the index pairs? (not have a solid solution now)\\

% list an algorithm for determining the data partitioning schemes for different join predicates\\

\textbf{Cost Model for Communications.}
\system~extends \oldsystem's~\cite{matfast} matrix data partitioner, and it naturally supports three matrix data partitioning schemes: \textit{Row}(``$r$''), \textit{Column}(``$c$''), and \textit{Broadcast}(``$b$''). The Broadcast scheme is only used for sharing a matrix of low dimensions, e.g., a single vector. Different matrix data partitioning schemes lead to significantly different communication overhead for join executions. Therefore, we introduce a cost model to evaluate the communication costs of various partitioning schemes for join operations on matrix data.

%Communication costs for different joins:
We design a communication cost model based on the join predicates. For cross-product, we have
\begin{align*}
C_{comm}(\mA \kron \mB)=\begin{cases}
    \hfil 0, & \text{if } s_{A/B}=b.\\
    (N-1)\min\{|\mA|, |\mB|\}, & \text{otherwise}.
  \end{cases}
\end{align*}
where $s_A$ and $s_B$ are the partitioning scheme of input matrix $\mA$ and $\mB$, and $N$ is the number of workers in the cluster. $|\mA|$ refers to the size of the Matrix $\mA$, i.e., $|\mA| = mn$ if $\mA$ is an $m$-by-$n$ dense matrix; and it means \texttt{nnz}$(\mA)$ if $\mA$ is sparse. The communication cost is 0 if one of the inputs has been broadcast to every worker in the cluster. This only applies to the case when either $\mA$ or $\mB$ is a matrix of tiny dimensions. When $\mA$ and $\mB$ are partitioned in Row/Column scheme, each partition of the smaller matrix has to be mapped to every worker. Therefore, it incurs a communication cost of $(N-1)\min\{|\mA|, |\mB|\}$.

For direct overlay, we have the following cost function,
\begin{align*}
  C_{comm}(\mA \Join_{\gamma, f} \mB) =\begin{cases}
    \frac{N-1}{N}\min\{|\mA|, |\mB|\}, & \text{if } (s_{A},s_{B})=\\
    &(r,c)\text{ or }(c, r).\\
   \hfil 0, & \text{otherwise}.
  \end{cases}
\end{align*}
It is clear that the direct overlay operation induces 0 communication overhead if one of the inputs is broadcast to all the workers in the cluster. Furthermore, there is no communication when both inputs are partitioned using the same scheme. Each worker receives matrix blocks with the same row/column block IDs from both inputs, and the join predicates are naturally satisfied. The communication overhead is only incurred when one of join operands is partitioned in Row scheme and the other is partitioned in Column scheme. To mitigate this partitioning scheme incompatibility, \system~repartitions the smaller matrix using the same data partitioning scheme from the larger matrix.

For transpose overlay, we have a similar cost function,
\begin{align*}
  C_{comm}(\mA \Join_{\gamma, f} \mB) =\begin{cases}
    \frac{N-1}{N}\min\{|\mA|, |\mB|\}, & \text{if } (s_{A},s_{B})=\\
    &(r,r) \text{ or }(c, c).\\
   \hfil 0, & \text{otherwise}.
  \end{cases}
\end{align*}
The cost model for a transpose overlay is very similar to that of the direct overlay case. The difference is that the communication overhead is introduced when two matrices are partitioned using the same scheme.

Table~\ref{tab:sinlge_dim_comm} summarizes the communication costs for joins on a single dimension. If any input matrix is broadcast to all the workers, there is no communication cost. We omit this case in  Table~\ref{tab:sinlge_dim_comm}.
Let us focus on the case when $\gamma=``RID_A=RID_B"$ and $(s_A, s_B) = (r,c)$. Figures~\ref{fig:join_cost_1_dim} illustrates that Matrix $\mA$ is partitioned in Row scheme and Matrix $\mB$ is partitioned in Column scheme. Suppose we have 3 workers in the cluster, i.e., $N=3$. Each square in the matrix is a block partition. The blocks with the same color are stored on the same worker. The join predicate requires that the entries sharing the same $RID$'s are joined together. There are two possible execution strategies based on the partitioning schemes of $\mA$ and $\mB$. Strategy I sends the blocks with the same $RID$ from $\mA$ to the workers which hold the joining blocks from $\mB$. For example, Worker $W_1$ sends all the blocks to Worker $W_2$ and $W_3$, since both $W_2$ and $W_3$ hold some joining blocks from $\mB$. Both $W_2$ and $W_3$ send the blocks in a similar manner. 
Each worker needs to send the blocks $(N\!-1)$ times to all the other workers. Thus, this strategy induces $(N\!-1)|\mA|$ communication cost.
Strategy II adopts a different policy by sending different blocks from $\mB$ to the same worker that holds the blocks with the same $RID$ from $\mA$. For example, the blocks with diagonal lines from $W_2$ and $W_3$ are sent to $W_1$ to satisfy the join predicate. As illustrated in Figure~\ref{fig:join_cost_1_dim}, all the blocks with diagonal lines introduce a communication cost of $\frac{N-1}{N}|\mB|$. Thus, the best communication cost is $\min\{(N-1)|\mA|, \frac{N-1}{N}|\mB|\}$ when $\gamma=``RID_A=RID_B"$ and $(s_A,s_B)=(r,c)$. 
The remaining entries in Table~\ref{tab:sinlge_dim_comm} can be computed with similar strategies.
Notice, the diagonal of Table~\ref{tab:sinlge_dim_comm} contains all 0's. This is because the partitioning schemes of both matrices happen to match the join predicate. %This is the ideal scenario where every worker computes the join locally without any communication.

\begin{table*}[!ht]
\centering
\scriptsize
\begin{tabular}{|c|c|c|c|c|} \hline
 & \multicolumn{4}{c|}{$(s_{A}, s_{B})$} \\  \hline
$\gamma$ & (r, r) & (r, c) & (c, r) & (c, c) \\ \hline
$RID_A=RID_B$ & 0 & $\min\{(N\!-1)|\mA|, \frac{N-1}{N}|\mB|\}$ & $\min\{\frac{N-1}{N}|\mA|, (N\!-1)|\mB|\}$ & $(N\!-1)\min\{|\mA|,  |\mB|\}$ \\ \hline 
$RID_A=CID_B$ & $\min\{(N\!-1)|\mA|, \frac{N-1}{N}|\mB|\}$ & 0 & $(N-1)\min\{|\mA|, |\mB|\}$ & $\min\{\frac{N-1}{N}|\mA|, (N\!-1)|\mB|\}$ \\ \hline
$CID_A=RID_B$ & $\min\{\frac{N-1}{N}|\mA|, (N\!-1)|\mB|\}$ & $(N-1)\min\{|\mA|,|\mB|\}$ & 0 & $\min\{(N\!-1)|\mA|, \frac{N-1}{N}|\mB|\}$ \\ \hline
$CID_A=CID_B$ & $(N-1)\min\{|\mA|,|\mB|\}$ & $\min\{\frac{N-1}{N}|\mA|, (N\!-1)|\mB|\}$ & $\min\{(N\!-1)|\mA|, \frac{N-1}{N}|\mB|\}$ & 0 \\ \hline
\end{tabular}
\captionof{table}{Communication cost of different D2D join predicates.}
%\vspace{-1em}
\label{tab:sinlge_dim_comm}
\end{table*}


\begin{figure}
\centering
\includegraphics[width=0.85\columnwidth]{./figs/join_comm}
\caption{Communication cost for D2D join.}
\vspace{-1em}
\label{fig:join_cost_1_dim}
\end{figure}

A join on entries has an identical cost function as a cross-product.
It is clear that the join execution incurs 0 communication cost if either $\mA$ or $\mB$ is partitioned in Broadcast scheme. For any other combination of partitioning schemes of $\mA$ and $\mB$, a worker needs to broadcast the smaller of the inputs to all the other workers. Hence, the communication cost is $(N-1)\min\{|\mA|, |\mB|\}$.

For a join on a single dimension and entries, Table~\ref{tab:sinlge_dim_val_comm} gives the communication costs for the various schemes. We use $\eta$ to denote the selectivity of entries that could match the row/column dimensions from the other matrix. Let us examine the cost function for $\gamma=``RID_A=val_B"$. %$(s_A, s_B)=(r,r)$, and $(s_A, s_B)=(c,r)$.
When $(s_A, s_B) = (r,r)$, there exist two strategies to evaluate the join. Strategy I requires each worker to send its own matrix blocks of $\mA$ to the other $(N-1)$ workers, since any worker may hold a block from $\mB$ that has matched entries with the row dimension. Broadcasting $\mA$ incurs a communication cost of $(N-1)|\mA|$.
Strategy II sends the matched entries from $\mB$ to each corresponding worker that holds the blocks of $\mA$. The selectivity indicates a total amount of $\eta_B|\mB|$ of matrix data is transferred. Thus, the communication cost would be $\min\{(N-1)|\mA|, \eta_B|\mB|\}$. 
For $(s_A, s_B) = (c,r)$, the only difference is that the selected matching entries from $\mB$ are sent to all the workers in the cluster, since $\mA$ is partitioned in Column scheme. The remaining entries in Table~\ref{tab:sinlge_dim_val_comm} can be computed in a similar manner.


\begin{table*}[!ht]
\centering
\scriptsize
\begin{tabular}{|c|c|c|c|c|} \hline
 & \multicolumn{4}{c|}{$(s_{A}, s_{B})$} \\  \hline
$\gamma$ & (r, r) & (r, c) & (c, r) & (c, c) \\ \hline
$RID_A=val_B$ & $\min\{(N\!-1)|\mA|,\eta_B|\mB|\}$ & $\min\{(N\!-1)|\mA|,\eta_B|\mB|\}$ & $\min\{(N\!-1)|\mA|,N\eta_B|\mB|\}$ & $\min\{(N\!-1)|\mA|,N\eta_B|\mB|\}$ \\ \hline 
$CID_A=val_B$ & $\min\{(N\!-1)|\mA|,N\eta_B|\mB|\}$ & $\min\{(N\!-1)|\mA|,N\eta_B|\mB|\}$ & $\min\{(N\!-1)|\mA|,\eta_B|\mB|\}$ & $\min\{(N\!-1)|\mA|,\eta_B|\mB|\}$ \\ \hline
$val_A=RID_B$ & $\min\{\eta_A|\mA|, (N\!-1)|\mB|\}$ & $\min\{N\eta_A|\mA|, (N\!-1)|\mB|\}$ & $\min\{\eta_A|\mA|, (N\!-1)|\mB|\}$ & $\min\{N\eta_A|\mA|,(N\!-1)|\mB|\}$ \\ \hline
$val_A=CID_B$ & $\min\{N\eta_A|\mA|, (N\!-1)|\mB|\}$ & $\min\{\eta_A|\mA|, (N\!-1)|\mB|\}$ & $\min\{N\eta_A|\mA|, (N\!-1)|\mB|\}$ & $\min\{\eta_A|\mA|, (N\!-1)|\mB|\}$ \\ \hline
\end{tabular}
\captionof{table}{Communication cost of different D2V and V2D join predicates.}
%\vspace{-1em}
\label{tab:sinlge_dim_val_comm}
\end{table*}

\textbf{Algorithm for Partitioning Scheme Assignment of Joins.}
Before we delve into the algorithm of partitioning scheme assignment for joins, we first discuss the cost function for converting distributed matrix data from one partitioning scheme to another.
Table~\ref{tab:convert_comm} illustrates the conversion costs, where $s_A$ is the partition scheme of an input, and $s'_A$ is the scheme for an output. $\xi$ denotes the case when the input data is randomly partitioned among all the workers in the cluster, e.g., round-robin. It introduces the communication cost of $|\mA|$ when re-partitioning Matrix $\mA$ from round-robin to Row/Column scheme. Broadcast scheme is more expensive and it costs $N|\mA|$, where each worker has a copy of all the matrix data.
\begin{table}[!ht]
\centering
\scriptsize
\begin{tabular}{|c|c|c|c|} \hline
 & \multicolumn{3}{c|}{$s'_{A}$} \\  \hline
$s_A$ & $r$ & $c$ & $b$ \\ \hline
$r$ & 0 & $\frac{N-1}{N}$|\mA| & $(N\!-1)|\mA|$ \\ \hline 
$c$ & $\frac{N-1}{N}|\mA|$ & 0 & $(N\!-1)|\mA|$ \\ \hline
$b$ & 0 & 0 & 0 \\ \hline
$\xi$ & $|\mA|$ & $|\mA|$ & $N|\mA|$ \\ \hline
\end{tabular}
\captionof{table}{Communication cost of converting partition schemes.}
\vspace{-1em}
\label{tab:convert_comm}
\end{table}

Given a join operation and input matrices $\mA$ and $\mB$, \system's data partitioner computes the best partition schemes for $\mA$ and $\mB$ by optimizing the following,
\begin{align*}
(s'_A,s'_B) \gets \argminl_{(s'_A,s'_B)} \; & \{C_{comm}(\mA \Join_{\gamma, f} \mB, s'_A, s'_B) \\
&+ C_{vt}(\mA, s_A \rightarrow s'_A) 
+ C_{vt}(\mB, s_B \rightarrow s'_B)\}.
\end{align*}
Function $C_{comm}(\mA \Join_{\gamma, f} \mB, s'_A, s'_B)$ computes the communication cost of the join according to our cost model when $\mA$ is partitioned in  Scheme $s_A$ and $\mB$ in Scheme $s_B$. Function $C_{vt}(\mA, s_A \rightarrow s'_A)$ computes the communication cost when converting $\mA$ from Scheme $s_A$ to $s'_A$. Essentially, the data partitioner adopts a grid-search strategy among all the possible combinations of partition schemes on the input matrices, and outputs the cheapest schemes for $\mA$ and $\mB$.

% \begin{algorithm}[!t]\small
% \KwIn{Join input $\mA, \mB$, predicate $\gamma$}
% \KwOut{Partitioning schemes for $\mA, \mB$}
% \If{$\gamma = \emptyset$ $||$ $\gamma = \{val_A = val_B\}$}
% {
% 	\If{$\mA.size \le \mB.size$}
%     {
%     	$\mA.scheme \gets $`b'
%     }
%     \Else
%     {
%     	$\mB.scheme \gets $`b'
%     }
% }
% \If{$\gamma$ is a direct overlay}
% {
% 	$\mA.scheme \gets$ `r'/`c'\\
%     $\mB.scheme \gets$ `r'/`c'
% }
% \If{$\gamma$ is a transpose overlay}
% {
% 	$\mA.scheme \gets$ `r'/`c'\\
%     $\mB.scheme \gets$ `c'/`r'
% }

% \caption{Partitioning scheme assignment for joins}
% \label{alg:join_partition}
% \end{algorithm}

==> figs/related-work.tex <==
\section{Related Work}
\label{sec:related-work}
We review related work of relational and matrix query processing and optimizations on matrix data. %in various systems.

\textbf{Matrix query processing on matrices:} There has been a long history of research on conducting efficient matrix computations in the high-performance computing~(HPC) community. Existing libraries provide efficient matrix operators, e.g., BLAS~\cite{blas} and LAPACK~\cite{lapack} (and its distributed variant ScaLAPACK~\cite{scalapack}). However, they lack support for sparse matrices, and are prone to machine failures. 

Recently, many systems have been proposed to support efficient matrix computations using Hadoop~\cite{hadoop} and Spark~\cite{Zaharia:spark}. These systems provide an easy-to-use interface on multiple matrix operations, e.g., HAMA~\cite{hama}, Mahout~\cite{mahout}, MLI~\cite{icdm13:mli}, MadLINQ~\cite{madlinq}, Cumulon~\cite{cumulon}, SystemML~\cite{icde11:systemml,vldb14:hybrid,vldb16:matrix,systemml-spark,spoof}, DMac \cite{sigmod15:DMac}, and \oldsystem~\cite{matfast}. Each system provides various optimization strategies for reducing memory consumption, computation and communication overhead. For example, SystemML~\cite{vldb16:matrix} adopts column encoding schemes and operations over compressed matrices to mitigate memory overhead when the original matrices are too large to fit in the available compute resources. \oldsystem~\cite{matfast} adopts a sampling-based approach to estimate the sparsity of matrix chain multiplications, and organizes distributed matrix partitions in a communication-efficient manner by leveraging matrix data dependencies. However, these systems focus on \textit{matrix-only} operations on big matrix data. None provides \textit{full-fledged} relational query processing on matrix data. \system~is built on \oldsystem, and provides optimized relational query processing on the distributed matrix data. %The relational operations cover a rich set of semantics on the matrix data for various application scenarios.
MATLANG~\cite{icdt18} examines matrix manipulation from the view of expressive power of database query language. It confirms the matrix operators provided by these systems are adequate for a wide range of applications.

\textbf{Matrix query processing on relations:}
A lot of work consider the problem of providing ML over relational data for specific ML algorithms. The assumption is the input dataset can be viewed as a join result on multiple tables. The so-called ``factorized machine learning'' tries to learn a model based on the de-normalized tables, without performing the join operation explicitly. For instance, \cite{regression-factor-join} aims at optimizing the linear regression model over factorized join tables. \cite{glm-factor} shows how to learn a generalized linear model over factorized join tables. Furthermore, \cite{join-feature-selection} discusses the cases when it is safe to conduct feature selection by avoiding key-foreign key joins to obtain features from all base tables. More recently, Morpheus~\cite{Morpheus} is proposed to conduct general linear algebra operations over factorized tables for popular ML algorithms. However, these systems rely on the  assumption that the input matrix is obtained from \textit{joins on multiple tables}, which is \textit{not} always the case for real-world applications, e.g., recommender systems.

\textbf{Relational query processing on matrices:}
The idea of building a universal array DBMS on multidimensional arrays for scientific and numerical applications has been explored for a long time. One of the most notable efforts is Rasdaman~\cite{rasdaman}.

Recently, there are several systems built from scratch with native support for linear algebra, such as SciDB~\cite{sigmod10:scidb,arraystore,skew-join} and TensorFlow~\cite{tensorflow}. %both of which support not only linear algebra, but also tensor algebra. %Tensorflow organizes operations into dataflow graphs, where nodes represent computations, and edges are the flow of data expressed using tensors. 
TensorFlow has limited support for distributed computation. The user has to manually map computation and data to each worker, since Tensorflow does not offer automatic work assignment~\cite{comparison-big-data-systems}. While Tensorflow is mainly designed for neural network models, it lacks well-defined relational operations on a matrix~(tensor).
SciDB supports the array data model, and adopts a share-nothing massively parallel processing~(MPP) architecture. SciDB provides a rich set of relational operations on the array data. However, it treats each array operator individually without tuning for a series of array operators. 

The MADlib project~\cite{vldb12:madlib} built analytics, including linear algebra functionality, on top of a database system. MADlib shows the potential of high-performance of linear algebra on top of a relational database. 
Recent extension on SimSQL~\cite{la-simsql} discusses the possibility of making a small set of changes to SQL for enabling a distributed, relational database engine to become a high-performance platform for distributed linear algebra. However, the extension does not cover the optimization on a series of mixed relational and matrix operations. Our work explores the potential to optimize the query execution pipeline by pushing relational operators below matrix operators, and computes costs for different plans. \system's query optimizer also takes into account the optimized data layout of join operands for communication-efficient executions.

==> figs/relational-ops.tex <==
\section{Relational operators on matrix data}
\label{sec:rel-algebra}

%In this section, we present the \textit{conceptual} schema of a matrix in terms of relational algebra. Based on the well-defined schema, we introduce basic relational operators on matrix data, i.e., selection, projection, aggregation, and join. Also, we study various optimization strategies for the relational operations over matrix data.

\noindent{\bf Relational Algebra for Matrix Data}: 
Relational algebra~\cite{Codd:1970} and its primitive operators operate over relations. All relational operators accept, as input, relations with properly defined schemas, and produce, as output, relations with certain schemas that are derived from the input schemas. 
To ensure expressive relational operators over matrix data, \system~ casts a general schema over all matrix data. 

\noindent
{\bf Relational Schema of a Matrix}:
\label{section:schema}
A matrix, say $\mA$, consists of two dimensional entries, $A_{ij}$. 
Each entry in a matrix resembles a tuple in a table with schema: \texttt{matrixA (RID, CID, val)},
where \texttt{RID} and \texttt{CID} are the row and column dimensions, respectively, and \texttt{val} is the value of the matrix entry. Attribute \texttt{val} may have its own schema as a tuple of multiple attributes. For simplicity, we only consider simple numerical values in the \texttt{val} attribute. In addition, \system~also maintains the dimension of the matrix in the system catalog, i.e., the number of rows and columns.
This schema specifies the logical structure of a matrix. However, it does \textit{not} reflect how the matrix is physically stored. For efficiency and storage considerations, a matrix is divided into ``blocks'', i.e., it is partitioned into smaller matrices that can be moved to specific compute nodes for high-performance local computations. Detailed physical storage of matrices is presented in Section~\ref{physical-storage-matrix}.

\noindent {\bf Relational Selection on Matrix Data}:
%Semantic of the selection operator on matrix data\\
Relational select~($\sigma$) selects matrix entries that qualify a certain predicate. 
We distinguish between selections on the dimensions, and the values of a matrix. 
A relational select is a unary operator of the form: 
$
\sigma_{\theta(RID, CID, val)}(\mA),
$
where $\theta$ is a propositional formula on the dimensions and entries of Matrix $\mA$. An atom in $\theta$ is defined as $v \varphi c$ or $c \varphi v$, where $v \in \{RID, CID, val\}$ is one of the dimensions or is the matrix entry, and $c$ is a constant, $\varphi \in \{<, \le, =, \neq, \ge, >\}$; and the logical expressions among atoms, i.e., $\land$~(and), $\lor$~(or), and $\neg$~(negation) expressions. A relational select on a matrix produces another matrix, perhaps with different dimensions. The dimensions depend on the predicate, e.g., the predicate $``RID=i"$ produces a matrix of a single row.

\noindent{\bf Selecting the Entries}:
A select over a matrix produces a matrix of the same dimension if the select predicate only involves Attribute $val$. 
The matrix entries that qualify the select predicate are preserved, and the remaining entries are set to 0.
The relational select on matrix entries does \emph{not} change the dimension of the input.  
Because the select predicate will be evaluated on the matrix entries, the input matrix to the select has to be computed fully before the select predicate is executed.
If a series of select predicates apply over a matrix, the following transformation rule applies:
\begin{equation} \label{rule:1}
\sigma_{\theta_1}(\sigma_{\theta_2}(\cdots(\sigma_{\theta_{k}}(\mA)))) = \sigma_{\theta_1 \land \theta_2 \land \cdots \land \theta_k}(\mA),
\end{equation}
where each $\theta_i$ is a predicate on the matrix entries.
%For other relational operations, the selection has to wait until the evaluation is completed, e.g., join and aggregation operations. 
%There is opportunity of optimizing a mixture of selections and projections. We discuss the optimization rules in the next section, after we introduce the projection operator.

\noindent
{\bf Relational Select on the Matrix Dimensions}: 
A select predicate can operate on the matrix dimensions to pick slices of a matrix according to the given row/column dimension value. 
For example, cross-validation~\cite{mlbook} is an ML technique to estimate how accurately a predicative model will perform in practice. Specifically, leave-\emph{one}-out cross-validation can be realized by selecting a single row from a training matrix as the test set. For simplicity, we only consider equality predicates on the matrix dimensions, 
% Formally, a relational project is a unary operator, written as 
% \[
% \sigma_{\theta(RID, CID)}(\mA),
% \]
% where $\tau$ is an equality predicate on the indices of a matrix, 
i.e., $\theta \in \{``RID=i"$, $``CID = j"$, $``RID=i \land CID=j"\}$.
The output of a select on the dimensions is a matrix with different dimensions than the input's, e.g., if the input is an $m\times n$ Matrix $\mA$, $\sigma_{RID = i}(\mA)$ is a $1\times n$ matrix whose entries are the $i$-th row of $\mA$.
Similarly, $\sigma_{CID = j}(\mA)$ is an $m\times 1$ matrix, and $\sigma_{RID = i \land CID = j}(\mA)$ outputs a $1\times 1$ matrix, whose entries are the $j$-th column and the $(i, j)$-th entry of $\mA$. %The projection definition guarantees a closure on the matrix data, i.e., the project always produces a new matrix.

%extended selection operation with the help of projection, e.g.,  selection on both value and index\\

%By introducing the projection operator, \system~is able to express selection on both entry values and indices. 
The select predicate can be composed of conditions on both dimensions and entries.
For instance, selecting all the entries whose values equal 10 from the 5-th row is expressed by $\sigma_{val = 10 \land RID = 5}(\mA)$.
Furthermore, in real-world ML applications, an empty column suggests no metrics have been observed for some feature. Removing empty columns will benefit the feature extraction procedure for better efficiency. Thus, we introduce two special predicates,
$
\sigma_{rows \neq 0}(\mA) \quad \text{and} \quad
\sigma_{cols \neq 0}(\mA).
$
The former excludes the rows that are all 0's, and the latter excludes the columns that are all 0's. These are important extensions to the select operator, because empty rows/columns usually do not contribute to matrix computations. 

\noindent
{\bf Optimizations for Selects over Dimensions}:
%A select predicate over dimensions exhibits potential opportunities for optimization. First, we discuss how to optimize a select when the input is composed of matrix operations. Next, we explore optimizations  when the input to the select involves multiple relational operations.
\system~supports matrix operations including transpose, matrix-scalar operation, matrix element-wise operation, and matrix-matrix multiplications. For matrix transpose, the transformation rules: $\sigma_{RID=i}(\mA^T) = (\sigma_{CID=i}(\mA))^T$ and $\sigma_{CID=j}(\mA^T) = (\sigma_{RID=j}(\mA))^T$ 
%\begin{align}
%\sigma_{RID=i}(\mA^T) &= (\sigma_{CID=i}(\mA))^T,\label{rule:2}\\
%\sigma_{CID=j}(\mA^T) &= (\sigma_{RID=j}(\mA))^T.\label{rule:3}
%\end{align}
reduce the computational costs significantly by avoiding the matrix transpose. It takes $O(n^2)$ operations to compute the matrix transpose on an $n \times n$ matrix. However, it only takes $O(n)$ operations for a typical select on a single dimension.

Similar rewrite rules apply to matrix-scalar and matrix element-wise operations. The following rules can be viewed as pushing the select below the matrix operations:
%\begin{align}
%\sigma_{RID=i}(\mA + \beta) &= \sigma_{RID=i}(\mA) + \beta, \label{rule:4}\\
%%\sigma_{RID=i}(\mA * \beta) &= \sigma_{RID=i}(\mA) * \beta, \label{rule:5}\\
%\sigma_{RID=i}(\mA \star \mB) &= \sigma_{RID=i}(\mA) \star \sigma_{RID=i}(\mB), \label{rule:6} 
%\end{align}
$\sigma_{RID=i}(\mA \star \mB) = \sigma_{RID=i}(\mA) \star \sigma_{RID=i}(\mB)$, 
where $\star \in \{+, *, /\}$. This rule
%~\ref{rule:4} 
also applies to matrix-scalar multiplications. We illustrate these transformation rules on the selects w.r.t. the row dimension. The rules apply to selections on the column dimension as well. The number of required operations drops from $O(n^2)$ to $O(n)$ by circumventing the intermediate matrix.
For matrix-matrix multiplications, we have $\sigma_{RID=i}(\mA \times \mB) = \sigma_{RID=i}(\mA) \times \mB$.
%\begin{align}
%\sigma_{RID=i}(\mA \times \mB) &= \sigma_{RID=i}(\mA) \times \mB, \label{rule:7}\\
%\sigma_{CID=j}(\mA \times \mB) &= \mA \times \sigma_{CID=j}(\mB). \label{rule:8}
%\end{align}
\begin{proof}%~\ref{rule:7})
%Let us derive Rule~\ref{rule:7} from the definition of matrix-matrix multiplication. 
Let $\mC = \mA \times \mB$, where $C_{ij} = \sum_k A_{ik} * B_{kj}$. $C_{i:}$ is the $i$-th row in Matrix $\mC$. Then, by definition, $C_{i:} = \sum_k A_{ik} * B_{k:}$, where $A_{ik}$ is the $(i, k)$-th entry from $\mA$, and $B_{k:}$ is $k$-th row from $\mB$. This can be viewed as the summation of each entry in the $i$-th row of $\mA$ multiplying with corresponding rows of $\mB$, i.e., $\mC_{i:} = \mA_{i:} \times \mB$.
\end{proof}
Analogously, the Rule: $\sigma_{CID=j}(\mA \times \mB) = \mA \times \sigma_{CID=j}(\mB)$
%~\ref{rule:8}
can be verified. It takes $O(n^3)$ operations for matrix-matrix multiplications, while a matrix-vector multiplication costs $O(n^2)$ operations. 
%These transformation rules are basic optimizing blocks for producing strategies when a selection is performed on multiple dimensions. For example, 
Furthermore, the rule:
%\begin{align}
%\sigma_{RID=i \land CID=j}(\mA \times \mB) = \sigma_{RID=i}(\mA) \times \sigma_{CID=j}(\mB), %\label{rule:9}
%\end{align}
$\sigma_{RID=i \land CID=j}(\mA \times \mB) = \sigma_{RID=i}(\mA) \times \sigma_{CID=j}(\mB)$
reduces the complexity from $O(n^3)$ (matrix-matrix multiplication) to $O(n)$ (vector inner-product).

% When the input matrix to the selection operator derives from a selection, we have the following transformation rule,
% \begin{align}
% \sigma_{\theta_1}(\sigma_{\theta_2}(\mA)) = \sigma_{\theta_2}(\sigma_{\theta_1}(\mA)).
% \end{align}
% As selection on dimensions usually generates a matrix of smaller dimensions compared to the original input, it is much cheaper to execute the selection operation before selection.

\noindent {\bf Projection on Matrix Data:}
Relational projection~($\Pi$) is used to select a subset of the attributes from the matrix. Formally, a projection on a matrix $\mA$ can be written as
\[
\Pi_{\tau(RID,CID,val)}(\mA),
\]
where $\tau$ is a subset of all the attributes $\{RID, CID, val\}$.
When \texttt{val} is a tuple, the predicate $\tau$ can be used to project only the interesting attributes from \texttt{val}'s. The produced matrix has the same dimension as $\mA$, and each entry contains the projected attributes from \texttt{val}.
Some applications may only be interested in the entries of a matrix, without caring about the dimensions, e.g., estimating the distribution of matrix entries. 
%The evaluation of projection on the entries is straight-forward. Each worker performs projection independently in a  parallel manner.
%Mingjie: why you mention the parallel computing here ? confused.
%Yongyang: I just want to mention the execution of this operation here. We can omit it here as other sections do not discuss the execution yet. I commented out the evaluation of projection on the entries.
A projection on the dimensions is less common, since the dimensions could be obtained from the matrix metadata directly.

The input to a projection can have different formats: a matrix expression of a series of matrix operations, or a matrix produced by relational operations. 
When a projection involves the entry, the input has to be evaluated before the projection. However, it is very efficient to evaluate a projection if it only involves dimensions of the input. No actual computation is required as the dimensionality can be inferred from the matrix operations or the relational operations. The only exception is the selecting the nonzero rows/columns. The nonzero selection has to be evaluated as it may change the dimension of the matrix.

%Mingjie: for the projection part, what is your observation ? or your contribution? I am little lost on this part. 
%Yongyang: For this part, we formalize the semantic definition of the projection operator. As we discussed above, this operator is not very common for matrix data. For a complete discussion of relational operators, I include it here.
%Mingjie: is here

\noindent {\bf Aggregation on Matrix Data:}
Traditionally, an aggregation is  defined on the columns of a relation with various aggregate functions, e.g., \texttt{sum} and \texttt{count}. The aggregation operator is also beneficial on matrix data, e.g., computing the average ratings of all the users in the user-movie rating database. %given that each row represents a user and each column represents a certain movie. 
The $(i,j)$-th entry in the user-movie rating matrix denotes the rating from $user_i$ on $movie_j$. This requires an average computation on the row dimension. Unlike relational data, aggregations on a matrix may occur in different dimensions. Formally, an aggregation is a unary operator, defined as
\[
\Gamma_{\rho,dim}(\mA),
\]
where $\rho$ is the name of the aggregate function, and $dim$ indicates the chosen dimension, i.e., $dim$ could be \emph{row}~(\emph{r}), \emph{column}~(\emph{c}), \emph{diagonal}~(\emph{d}), or \emph{all}~({\emph{a}}).
Specially, \system~supports various aggregate functions, $\rho \in \{\texttt{sum}, \texttt{nnz}$, $\texttt{avg}, \texttt{max}, \texttt{min}\}$. We introduce each aggregate function and corresponding optimizations in this section.

%matrix has 2 dims; extended to row agg, col agg, diag agg, mat agg.
\noindent {\bf \texttt{Sum()} Aggregate:}
%Variants along different dimensions, e.g., rowSum, colSum, sum, diagSum\\
For \texttt{sum} aggregation, \system~supports four different variants, $\Gamma_{\texttt{sum}, r/c/d/a}(\mA)$. 
%$\Gamma_{\texttt{sum}, c}$, $\Gamma_{\texttt{sum}, d}$, and $\Gamma_{\texttt{sum},a}$. 
We first introduce their definitions, then discuss optimization strategies. Given an $m$-by-$n$ Matrix $\mA$, $\Gamma_{\texttt{sum}, r}(\mA)$ produces a $m$-by-1 matrix, or a column vector, whose $i$-th entry computes the summation along the $i$-th row of $\mA$. Similarly,
$\Gamma_{\texttt{sum}, c}(\mA)$ generates a 1-by-$n$ matrix, or a row vector, which computes the summations of entries along the column direction. $\Gamma_{\texttt{sum}, d}(\mA)$ is defined only if $m=n$ for square matrices, which is also called the \emph{trace} of a square matrix. The trace is simply a 1-by-1 matrix, or a scalar value. Finally, $\Gamma_{\texttt{sum},a}(\mA)$ computes the summation of all the entries.

%Sum pushdown on matrix operators
We first present transformation rules for optimizing \texttt{sum} aggregation when the input consists of various matrix operations. If the input is a matrix transpose, we have
\begin{align}
\Gamma_{\texttt{sum}, r/c}(\mA^T) &= (\Gamma_{\texttt{sum}, c/r}(\mA))^T, \label{rule:11}\\
%\Gamma_{\texttt{sum}, c}(\mA^T) &= \Gamma_{\texttt{sum}, r}(\mA)^T, \label{rule:12}\\
\Gamma_{\texttt{sum}, d/a}(\mA^T) &= \Gamma_{\texttt{sum}, d/a}(\mA), \label{rule:12}
%\Gamma_{\texttt{sum},a}(\mA^T) &= \Gamma_{\texttt{sum},a}(\mA). \label{rule:14}
\end{align}
By pushing a \texttt{sum} aggregation before a matrix transpose, \system~computes the transpose on a matrix of smaller dimensions. For trace and all entry summation, the evaluation of the transpose can be avoided.

For matrix-scalar operations, we can derive the following transformation rules,
\begin{align}
\Gamma_{\texttt{sum}, r/c/a}(\mA + \beta) &= \Gamma_{\texttt{sum}, r/c/a}(\mA) + \beta n/\beta m/\beta mn, \label{rule:13}\\
%\Gamma_{\texttt{sum}, c}(\mA + \beta) &= \Gamma_{\texttt{sum}, c}(\mA) + \beta m, \label{rule:14}\\
\Gamma_{\texttt{sum}, d}(\mA + \beta) &= \Gamma_{\texttt{sum}, d}(\mA) + \beta n, \label{rule:15}\\
%\Gamma_{\texttt{sum},a}(\mA + \beta) &= \Gamma_{\texttt{sum},a}(\mA) + \beta m n, \label{rule:16}\\
\Gamma_{\texttt{sum}, \cdot}(\mA * \beta) &= \Gamma_{\texttt{sum}, \cdot}(\mA) * \beta, \label{rule:17}
\end{align}
where Rule~\ref{rule:15} only holds for square matrices, i.e., $m=n$. For matrix-scalar multiplications, similar rules apply when the aggregation is executed along the column direction, diagonal direction, and the entire matrix.

For matrix element-wise operations, only the matrix element-wise addition has a compatible transformation rule for \texttt{sum} aggregations.
\begin{align}
\Gamma_{\texttt{sum}, \cdot}(\mA + \mB) = \Gamma_{\texttt{sum}, \cdot}(\mA) + \Gamma_{\texttt{sum}, \cdot}(\mB). \label{rule:18}
\end{align}
Though Rule~\ref{rule:18} does not change the computation overhead, it circumvents storing the intermediate sum matrix $\mA+\mB$, alleviating memory footprint.

For matrix-matrix multiplications, we derive efficient transformation rules to compute the \texttt{sum} aggregations,
\begin{align}
\Gamma_{\texttt{sum}, r}(\mA \times \mB) &= \mA \times \Gamma_{\texttt{sum}, r}(\mB), \label{rule:19}\\
\Gamma_{\texttt{sum}, c}(\mA \times \mB) &= \Gamma_{\texttt{sum}, c}(\mA) \times \mB, \label{rule:20}\\
\Gamma_{\texttt{sum}, a}(\mA \times \mB) &= \Gamma_{\texttt{sum}, c}(\mA) \times \Gamma_{\texttt{sum}, r}(\mB), \label{rule:21}\\
\Gamma_{\texttt{sum}, d}(\mA \times \mB) &= \Gamma_{\texttt{sum}, a}(\mA^T * \mB) = \Gamma_{\texttt{sum}, a}(\mA * \mB^T). \label{rule:22}
\end{align}
\begin{proof}(Rule~\ref{rule:19})
%Let us derive Rule~\ref{rule:19} from the definition. 
Let $\mC = \mA \times \mB$, where $C_{ij} = \sum_{k}A_{ik} * B_{kj}$. Let the column Vector $\vy = \Gamma_{\texttt{sum}, r}(\mC)$. Therefore,
\[
y_i = \sum_j C_{ij}
=\sum_j \sum_k A_{ik} * B_{kj}
%&= \sum_k A_{ik} * \left(\sum_j B_{kj}\right)\\
= \sum_k A_{ik} * b_k,
\]
where Vector $\vb = \Gamma_{\texttt{sum}, r}(\mB)$.
It is clear that the derivation in the matrix format, $\vy = \mA \times \vb$, which is \emph{exactly} Rule~\ref{rule:19}.
\end{proof}
Similar derivations also apply to Rule~\ref{rule:20} and \ref{rule:21}. For Rule~\ref{rule:22}, both input matrices are required to be square. 
\begin{proof}(Rule~\ref{rule:22})
Let us write Matrix $\mA$ in terms of rows, and Matrix $\mB$ in terms of columns,
\[
\mA =
\begin{bmatrix}
\va_1^T \\ \vdots \\ \va_n^T
\end{bmatrix}, \quad
\mB = 
\begin{bmatrix}
\vb_1 &\cdots &\vb_n
\end{bmatrix}.
\]
Therefore, the matrix-matrix multiplication can be represented by Vector $\va_i$'s and $\vb_i$'s.
\[
\mA \times \mB = 
\begin{bmatrix} 
    \va_1^T\vb_1 & \dots & \va_1^T\vb_n \\
    \vdots & \ddots & \vdots \\
    \va_n^T\vb_1 & \dots & \va_n^T\vb_n 
\end{bmatrix}
\]
The trace of $\mA \times \mB$ can be  computed as $\Gamma_{\texttt{sum}, d}(\mA \times \mB) = \sum_{i=1}^n \va_i^T \times \vb_i$.
The transpose of $\mA$ is represented as,
\[
\mA^T = 
\begin{bmatrix}
\va_1 &\cdots &\va_n
\end{bmatrix},
\]
and the matrix element-wise multiplication is computed as,
\[
\mA^T * \mB = 
\begin{bmatrix}
\va_1*\vb_1 &\cdots &\va_n * \vb_n
\end{bmatrix}.
\]
When conducting the all entry \texttt{sum} aggregation, it is essentially to compute the inner-product of corresponding vector pairs, i.e., $\Gamma_{\texttt{sum},a}(\mA^T * \mB) = \sum_{i=1}^n \va_i^T \times \vb_i$. The second half of Rule~\ref{rule:22} can be verified in a similar manner.
\end{proof}

The computation complexity is usually $O(n^3)$ for $n$-by-$n$ square matrix-matrix multiplications. By leveraging matrix element-wise multiplication and matrix transpose, the complexity is reduced to $O(n^2)$.

Unfortunately, equivalent transformation rules do not apply when the input involves a relational selection or projection. For general selection condition $\theta$ and projection predicate $\tau$, 
\begin{align}
\Gamma_{\texttt{sum}, \cdot}(\sigma_\theta(\mA)) &\neq \sigma_\theta(\Gamma_{\texttt{sum}, \cdot}(\mA)), \label{rule:23}\\
\Gamma_{\texttt{sum},\cdot}(\Pi_\tau(\mA)) &\neq \Pi_\tau(\Gamma_{\texttt{sum},\cdot}(\mA)). \label{rule:24}
\end{align}
However, there exist valid transformation rules if the \texttt{sum} dimension happens to match with the predicate of the selection, e.g., $\Gamma_{\texttt{sum}, r}(\sigma_{RID=i}(\mA)) = \sigma_{RID=i}(\Gamma_{\texttt{sum}, r}(\mA))$. Swapping the execution order of \texttt{sum} aggregation and projection leads to the same result. Pushing a selective relational operation below a matrix operation is beneficial, as it could reduce the dimension of the matrix.



\noindent {\bf \texttt{Count()} Aggregate:}
For relational data, the \texttt{count} aggregate function computes the number of tuples that satisfy a certain criteria. For matrix data, the \texttt{count} function is usually interpreted as computing the number of nonzeros~(\texttt{nnz}). This function is quite useful for optimizing matrix computations, e.g., sparsity estimation for sparse matrix chain multiplications~\cite{matfast}.
Similar to \texttt{sum} aggregation, \system~supports four \texttt{count} variants, $\Gamma_{\texttt{nnz},r/c/d/a}(\mA)$. %$\Gamma_{\texttt{nnz}, c}$, $\Gamma_{\texttt{nnz}, d}$, and $\Gamma_{\texttt{nnz}, a}$. 
The output of each function is defined as its counterpart of  the \texttt{sum} function correspondingly.

%Variants along different dimensions, e.g., rowNNZ, colNNZ, NNZ, diagNNZ\\
We present equivalent transformation rules for optimizing \texttt{count} aggregations when the input is composed of various matrix operations. For matrix transpose, we have
\begin{align}
\Gamma_{\texttt{nnz}, r/c}(\mA^T) &= (\Gamma_{\texttt{nnz}, c/r}(\mA))^T, \label{rule:25}\\
%\Gamma_{\texttt{nnz}, c}(\mA^T) &= \Gamma_{\texttt{nnz}, r}(\mA)^T, \label{rule:28}\\
\Gamma_{\texttt{nnz}, d/a}(\mA^T) &= \Gamma_{\texttt{nnz}, d/a}(\mA). \label{rule:27}
%\Gamma_{\texttt{nnz}, a}(\mA^T) &= \Gamma_{\texttt{nnz}, a}(\mA)^T. \label{rule:30}
\end{align}
These rules push a \texttt{count} aggregation below a matrix transpose. The postponed matrix transpose is executed on a smaller matrix, e.g., a vector, avoiding $O(n^2)$ computations for the matrix transpose.

For matrix-scalar operations, let $\mA$ be an $m$-by-$n$ matrix, and scalar $\beta \neq 0$. We denote $\ve(n)$ to be an all-one column vector of length $n$. The following  rules hold for an input that involves matrix-scalar operations,
\begin{align}
\Gamma_{\texttt{nnz}, r}(\mA + \beta) &= \ve(m) * n, \label{rule:27}\\
\Gamma_{\texttt{nnz}, c}(\mA + \beta) &= \ve(n)^T * m, \label{rule:28}\\
\Gamma_{\texttt{nnz}, d}(\mA + \beta) &= n, \label{rule:29}\\
\Gamma_{\texttt{nnz}, a}(\mA + \beta) &= mn, \label{rule:30}\\
\Gamma_{\texttt{nnz}, \cdot}(\mA * \beta) &= \Gamma_{\texttt{nnz}, \cdot}(\mA). \label{rule:31}
\end{align}
By assuming the constant $\beta \neq 0$, the number of zeros is not altered for matrix-scalar multiplications. For the matrix-scalar addition, the output does not depend on the entries in $\mA$, which only requires the dimensions to conduct the computation.

For matrix element-wise operations, only the division operator works friendly with \texttt{count} aggregation.
\begin{align}
\Gamma_{\texttt{nnz}, \cdot}(\mA / \mB) = \Gamma_{\texttt{nnz}, \cdot}(\mA) \label{rule:32}
\end{align}
Rule~\ref{rule:32} indicates the matrix element-wise division preserves the number of nonzeros of the numerator matrix. Unfortunately, such convenient transformation rules do not apply to other matrix element-wise operators and matrix-matrix multiplications.

For an input consisting of relational selections and projections, Rule~\ref{rule:23} and \ref{rule:24} can be extended too. It is impossible to swap the execution order of a \texttt{count} aggregation and a selection for a correct output. It is only valid to swap the execution order of a \texttt{count} aggregation and a selection when both work on the same dimension, e.g., $\Gamma_{\texttt{nnz}, c}(\sigma_{CID=j}(\mA)) = \sigma_{CID=j}(\Gamma_{\texttt{nnz}, c}(\mA))$.


\noindent {\bf \texttt{Avg()} Aggregate:}
%Variants along different dimensions, e.g., rowAvg, colAvg, avg, diagAvg\\
The \texttt{avg} aggregate function computes the average statistic on a matrix in a certain dimension. \system~supports four different variants, $\Gamma_{\texttt{avg}, r/c/d/a}(\mA)$. %$\Gamma_{\texttt{avg}, c}$, $\Gamma_{\texttt{avg}, d}$, and $\Gamma_{\texttt{avg}, a}$. 
The output of each \texttt{avg} aggregate function is defined as its counterpart of the \texttt{sum} aggregation correspondingly. The \texttt{avg} aggregation can be viewed as a compound operator from a \texttt{sum} and a \texttt{count} aggregations. Formally, any \texttt{avg} aggregation can be computed as
\[
\Gamma_{\texttt{avg}, \cdot}(\mA) = \Gamma_{\texttt{sum},\cdot}(\mA) / \Gamma_{\texttt{nnz}, \cdot}(\mA).
\]
Therefore, optimizing an \texttt{avg} aggregation can leverage all the transformation rules we have explored for \texttt{sum} and \texttt{count} aggregations.
\system's optimizer automatically invokes query planning for corresponding \texttt{sum} and \texttt{count} aggregations when generating an execution plan for an \texttt{avg} aggregation.


%Avg pushdown on matrix operators

\noindent {\bf \texttt{Max()}/\texttt{Min()} Aggregate:}
%Variants along different dimensions, e.g., rowMax, colMax, max, diagMax\\
The \texttt{max}~(or \texttt{min}) aggregation is used to obtain the extreme values from a matrix, which serves as an important building block for anomaly detection~\cite{anomaly-detection-survey} in data mining applications. Naturally, \system~supports four \texttt{max}~(or \texttt{min}) variants, $\Gamma_{\texttt{max}/\texttt{min}, r/c/d/a}(\mA)$. %$\Gamma_{\texttt{max}/\texttt{min}, c}$, $\Gamma_{\texttt{max}/\texttt{min}, d}$, and $\Gamma_{\texttt{max}/\texttt{min}, a}$. 
The output of each aggregation is defined as its counterpart of the \texttt{sum} aggregation correspondingly.
The transformation rules for optimizing \texttt{max}~(or \texttt{min}) aggregation can be derived as follows,
\begin{align}
\Gamma_{\texttt{max}/\texttt{min}, r/c}(\mA^T) &= (\Gamma_{\texttt{max}/\texttt{min}, c/r}(\mA))^T, \label{rule:33}\\
\Gamma_{\texttt{max}/\texttt{min}, d/a}(\mA^T) &= \Gamma_{\texttt{max}/\texttt{min}, d/a}(\mA), \label{rule:34} \\
\Gamma_{\texttt{max}/\texttt{min}, \cdot}(\mA + \beta) &= \Gamma_{\texttt{max}/\texttt{min}, \cdot}(\mA) + \beta, \label{rule:35}\\
\Gamma_{\texttt{max}/\texttt{min}, \cdot}(\mA * \beta) &= \Gamma_{\texttt{max}/\texttt{min}, \cdot}(\mA) * \beta \quad (\beta > 0), \label{rule:36}\\
\Gamma_{\texttt{max}/\texttt{min}, \cdot}(\mA * \beta) &= \Gamma_{\texttt{min}/\texttt{max}, \cdot}(\mA) * \beta \quad (\beta < 0). \label{rule:37}
\end{align}
We assume the constant scalar $\beta \neq 0$. When $\beta < 0$, the optimizer computes the \texttt{min}/\texttt{max} aggregation instead for avoiding the intermediate matrix $\mA * \beta$. For matrix element-wise operations and matrix-matrix multiplications, \textit{no} general rules apply.
For example, $\Gamma_{\texttt{min}, r}([1,1,2] + [3,0.5,0]) =\Gamma_{\texttt{min}, r}([4,1.5,2]) =1.5$, which could only be evaluated after computing the sum of the two matrices.
For an input consisting of relational selections and projections, it is only valid to swap the execution order of a \texttt{max}/\texttt{min} aggregation and selection when both work on the same dimensions.

%max pushdown on matrix operators

% \subsubsection{\texttt{Min()} on matrix data}
% Variants along different dimensions, e.g., rowMin, colMin, min, diagMin\\

% min pushdown on matrix operators

\input{join.tex}


